More cat than cute? Interpretable Prediction of Adjective-Noun Pairs

The increasing availability of affect-rich multimedia resources has bolstered interest in understanding sentiment and emotions in and from visual content. Adjective-noun pairs (ANP) are a popular mid-level semantic construct for capturing affect via visually detectable concepts such as "cute dog" or "beautiful landscape". Current state-of-the-art methods approach ANP prediction by considering each of these compound concepts as individual tokens, ignoring the underlying relationships in ANPs. This work aims at disentangling the contributions of the `adjectives' and `nouns' in the visual prediction of ANPs. Two specialised classifiers, one trained for detecting adjectives and another for nouns, are fused to predict 553 different ANPs. The resulting ANP prediction model is more interpretable as it allows us to study contributions of the adjective and noun components. Source code and models are available at https://imatge-upc.github.io/affective-2017-musa2/ .

==> 8_annex.tex <==
\begin{table*}[htp]
\centering
\caption{Examples of ANP Contribution Table}
\label{table:coocurring_concepts}
\begin{tabular}{@{}lccclccc@{}}
\toprule
\multirow{17}{*}{Add Image} & \multicolumn{3}{c}{\textbf{ANP Name}}                                       & \multirow{17}{*}{Add Image} & \multicolumn{3}{c}{\textbf{ANP Name}}                                      \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{3}{c}{\textbf{Accuracy}}                                                   &     & \multicolumn{3}{c}{\textbf{Accuracy}}                                                                                   \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
  & \multicolumn{1}{l|}{\textbf{Network}}         & \textbf{top-1}      & \textbf{top-5}    &     & \multicolumn{1}{l|}{\textbf{Network}}         & \multicolumn{1}{l}{\textbf{top-1}} & \multicolumn{1}{l}{\textbf{top-5}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{l|}{\textbf{ANPnet}}      & XX.XX\%             & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{ANPnet}}      & XX.XX\%             				& XX.XX\%                           \\
  & \multicolumn{1}{l|}{\textbf{AdjNet}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{AdjNet}}          & XX.XX\%                            & XX.XX\%         \\
  & \multicolumn{1}{l|}{\textbf{NounNet}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{NounNet}}          & XX.XX\%                            & XX.XX\%         \\
  \cmidrule(lr){2-4} \cmidrule(l){6-8}
  
  & \multicolumn{3}{c}{\textbf{ANR (top-5)}}    								&     & \multicolumn{3}{c}{\textbf{ANR (top-5)}}                \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{l|}{\textbf{Correct ANPs}}      & XX.XX\%             & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{Correct ANPs}}      & XX.XX\%             				& XX.XX\%                           \\
  & \multicolumn{1}{l|}{\textbf{All top-5 ANP}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{All top-5 ANP}}          & XX.XX\%                            & XX.XX\%         \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{3}{c}{\textbf{Semantic Contributions}}                                     &      & \multicolumn{3}{c}{\textbf{Semantic Contributions}}                                                                     \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{c|}{\textbf{top-5 adjective}} & \multicolumn{2}{c}{\textbf{top-5 noun}} &      & \multicolumn{1}{c|}{\textbf{top-5 adjective}} & \multicolumn{2}{c}{\textbf{top-5 noun}}                                 \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
  & \multicolumn{1}{c|}{xxx}                & \multicolumn{2}{c}{xxx}           	&      & \multicolumn{1}{c|}{xxx}                    & \multicolumn{2}{c}{xxx}                                               \\
  & \multicolumn{1}{c|}{xxx}                  	  & \multicolumn{2}{c}{xxx}                &      & \multicolumn{1}{c|}{xxx}                  & \multicolumn{2}{c}{xxx}                                                \\
  & \multicolumn{1}{c|}{xxx}                    & \multicolumn{2}{c}{xxx}                 &      & \multicolumn{1}{c|}{xxx}                  & \multicolumn{2}{c}{xxx}                                                 \\
  & \multicolumn{1}{c|}{xxx}                      & \multicolumn{2}{c}{xxx}           &      & \multicolumn{1}{c|}{xxx}                     & \multicolumn{2}{c}{xxx}                                           \\
  & \multicolumn{1}{c|}{xxx}                      & \multicolumn{2}{c}{xxx}                 &      & \multicolumn{1}{c|}{xxx}                   & \multicolumn{2}{c}{xxx}                                                \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} \\
  
 
 
 \toprule
\multirow{17}{*}{Add Image} & \multicolumn{3}{c}{\textbf{ANP Name}}                                       & \multirow{17}{*}{Add Image} & \multicolumn{3}{c}{\textbf{ANP Name}}                                      \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{3}{c}{\textbf{Accuracy}}                                                   &     & \multicolumn{3}{c}{\textbf{Accuracy}}                                                                                   \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
  & \multicolumn{1}{l|}{\textbf{Network}}         & \textbf{top-1}      & \textbf{top-5}    &     & \multicolumn{1}{l|}{\textbf{Network}}         & \multicolumn{1}{l}{\textbf{top-1}} & \multicolumn{1}{l}{\textbf{top-5}} \\ 
  \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{l|}{\textbf{ANPnet}}      & XX.XX\%             & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{ANPnet}}      & XX.XX\%             				& XX.XX\%                           \\
  & \multicolumn{1}{l|}{\textbf{AdjNet}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{AdjNet}}          & XX.XX\%                            & XX.XX\%         \\
  & \multicolumn{1}{l|}{\textbf{NounNet}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{NounNet}}          & XX.XX\%                            & XX.XX\%         \\
  \cmidrule(lr){2-4} \cmidrule(l){6-8}
  
  & \multicolumn{3}{c}{\textbf{ANR (top-5)}}    								&     & \multicolumn{3}{c}{\textbf{ANR (top-5)}}                \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{l|}{\textbf{Correct ANPs}}      & XX.XX\%             & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{Correct ANPs}}      & XX.XX\%             				& XX.XX\%                           \\
  & \multicolumn{1}{l|}{\textbf{All top-5 ANP}}            & XX.XX\%            & XX.XX\%            &      & \multicolumn{1}{l|}{\textbf{All top-5 ANP}}          & XX.XX\%                            & XX.XX\%         \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{3}{c}{\textbf{Semantic Contributions}}                                     &      & \multicolumn{3}{c}{\textbf{Semantic Contributions}}                                                                     \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}
  & \multicolumn{1}{c|}{\textbf{top-5 adjective}} & \multicolumn{2}{c}{\textbf{top-5 noun}} &      & \multicolumn{1}{c|}{\textbf{top-5 adjective}} & \multicolumn{2}{c}{\textbf{top-5 noun}}                                 \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
  & \multicolumn{1}{c|}{xxx}                & \multicolumn{2}{c}{xxx}           	&      & \multicolumn{1}{c|}{xxx}                    & \multicolumn{2}{c}{xxx}                                               \\
  & \multicolumn{1}{c|}{xxx}                  	  & \multicolumn{2}{c}{xxx}                &      & \multicolumn{1}{c|}{xxx}                  & \multicolumn{2}{c}{xxx}                                                \\
  & \multicolumn{1}{c|}{xxx}                    & \multicolumn{2}{c}{xxx}                 &      & \multicolumn{1}{c|}{xxx}                  & \multicolumn{2}{c}{xxx}                                                 \\
  & \multicolumn{1}{c|}{xxx}                      & \multicolumn{2}{c}{xxx}           &      & \multicolumn{1}{c|}{xxx}                     & \multicolumn{2}{c}{xxx}                                           \\
  & \multicolumn{1}{c|}{xxx}                      & \multicolumn{2}{c}{xxx}                 &      & \multicolumn{1}{c|}{xxx}                   & \multicolumn{2}{c}{xxx}                                                \\ \cmidrule(lr){2-4} \cmidrule(l){6-8}

\end{tabular}
\end{table*}

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges
		
